Belief Revision: The Adaptability of Large Language Models Reasoning

The capability to reason from text is crucial for real-world NLP applications. Real-world scenarios often involve incomplete or evolving data. In response, individuals update their beliefs and understandings accordingly. However, most existing evaluations assume that language models (LMs) operate with consistent information. We introduce Belief-R, a new dataset designed to test LMs' belief revision ability when presented with new evidence. Inspired by how humans suppress prior inferences, this task assesses LMs within the newly proposed delta reasoning ($\Delta R$) framework. Belief-R features sequences of premises designed to simulate scenarios where additional information could necessitate prior conclusions drawn by LMs. We evaluate $\sim$30 LMs across diverse prompting strategies and found that LMs generally struggle to appropriately revise their beliefs in response to new information. Further, models adept at updating often underperformed in scenarios without necessary updates, highlighting a critical trade-off. These insights underscore the importance of improving LMs' adaptiveness to changing information, a step toward more reliable AI systems.

==> anli.tex <==

% \begin{table}
% \centering
% \resizebox{0.9\columnwidth}{!}{%
% \begin{tabular}{lc}
% \toprule
% \multicolumn{1}{c}{\textbf{Error Types}} & \textbf{Ratio} \\
% \midrule
% Context misunderstanding & 1.59\% \\
% Not considering all of the premises & 61.90\% \\
% Mistake in consideration & 17.46\% \\
% Wrong mention of final answer & 6.35\% \\
% Both options are equally plausible & 9.52\% \\
% Dataset imperfection & 3.17\% \\
% \bottomrule
% \end{tabular}%
% }
% \caption{
% Error analysis on $\alpha$NLI task on randomly sampled inaccurate GPT-3.5 inferences in the test set. Taking the chain of thoughts as the elicited reasoning steps, we found that $\sim$60\% of the inferences do not actually consider all of premises in contexts, and $\sim$20\% of them. Here, dataset imperfection error refers to a wrong ground truth assignment and a typo in the dataset.
% }
% \label{tab:error_analysis_anli}
% \end{table}


% Despite their remarkable abilities, large language models have known to exhibit limitations in handling non-monotonic reasoning tasks. Here we consider the abduction task, a task of reasoning or inferencing to the best explanation that requires evaluating commonsense implications in a nonmonotonic way~\cite{brewka1997nonmonotonic}. We showcase this limitation by revisiting the abductive reasoning task and performing manual error analysis on the model's inferences. We randomly select 63 inaccurate GPT-3.5 inferences on the test set of $\alpha$NLI~\cite{bhagavatula2020abductive}. The dataset contains questions each with two observations that happens one before the other and two potential explanations. In this case, reasoners are being prompted to infer: "Which of the explanation is the most plausible to happen between them?". 

% We perform the inferences following~\citet{kojima2022large} by adding "let's think step by step" to the end of each question. Additionally, we follow~\citet{yao2022react} and prompt the model to format their final output, for us to perform automatic evaluation over them. We take the chain of thoughts as the elicited reasoning steps, and manually label their error types. From the summarized results in Table~\ref{tab:error_analysis_anli} we can observe that most errors happen when in its inferences through chain of thought, the model does not consider all of the premises in the context. When the model have made plausible inferences, it ignore the presence of more plausible options in the context, and tend to not retract its conclusions. While the behaviour is not unique only to the error cases, we conjecture that this behaviour indicates lack of nonmonotonic reasoning capabilities.

% % While existing research predominantly targets enhancing model performance on the tasks through multiple approaches, there is still a lack of 
% This observation motivate us to deepen our understanding about the model's nonmonotonic reasoning capability, 
% % perform in-depth investigations,
% particularly in model's behavior when confronted with information that might necessitate adjustments or reconsideration of their conclusions. 
% % We first aim to . 
% We put emphasis in the consideration process and develop datasets
% that involves logically valid inferences with
% % with various types of plausible inferences: logically valid or contextual inferences, and
% various strengths of the additional information introduced in the context. In this setting, we further analyze and evaluate model's ability to detect conflicts or changes, re-evaluate its conclusions, and revise or retract its conclusions. We highlight the differentiaton of our dataset in Table \ref{tab:dataset_comparison}. \placeholder{Further, we then focus on improving model's nonmonotonic inferences with the new and existing public datasets that necessitate nonmonotonic reasoning capabilities.}

% % The dataset lacks a designated "trigger" for evaluating conclusion adjustment/revisions, which is essential for testing NMR capabilities. It might be worthwhile to highlight that existing LLM use cases employing nonmonotonic reasoning, such as abductive reasoning, do not readily exhibit errors pertaining to NMR (or focuses on the core component NMR capabilities). This observation points to a potential oversight in current methodologies.

% % Furthermore, nonmonotonic reasoning system also requires the capacity to deal with uncertainties and inconsistencies in knowledge without leading to a collapse in reasoning capability. 
% %  In this work, we focus language model capability to dynamically adapt their inferences in response to new insights or evidence.

% % \subsection{Components}
% % We follow \citet{sep-logic-nonmonotonic} and adopt the devised framework to capture and represent the \textit{defeasible inference}. 
